Arcula: A Secure Hierarchical Deterministic Wallet for Multi-asset Blockchains

This work presents Arcula, a new design for hierarchical deterministic wallets that brings identity-based addresses to the blockchain. Arcula is built on top of provably secure cryptographic primitives. It generates all its cryptographic secrets from a user-provided seed and enables the derivation of new public keys based on the identities of users, without requiring any secret information. Unlike other wallets, it achieves all these properties while being secure against privilege escalation. We formalize the security model of hierarchical deterministic wallets and prove that an attacker compromising an arbitrary number of users within an Arcula wallet cannot escalate his privileges and compromise users higher in the access hierarchy. Our design works out-of-the-box with any blockchain that enables the verification of signatures on arbitrary messages. We evaluate its usage in a real-world scenario on the Bitcoin Cash network.

==> chain.tex <==
\section{Deterministic Wallets through Chain-Based Key Assignment}\label{sec:deterministic_wallets_through_chain_based_key_assigment}

\subsection{Chain-based Hierarchical Key Assignment schemes}\label{sub:chain_based_hierarchical_key_assignment_schemes}
After reviewing the existing literature in Hierarchical Key Assignment schemes we found that there exists a family of schemes, that:
\begin{itemize}
    \item Is provably secure under key indistinguishability.
    \item Does not require storing any public information.
    \item Provides efficient key derivation in both time and space.
\end{itemize}
Such schemes are based on chain or tree partitioning and have been first described by J. Crampton \emph{et al.}~\cite{crampton2010} in 2010.
The informal intuition behind these schemes is to partition any arbitrary hierarchy (encoded as a graph representing the partially ordered set, \emph{i.e.}, the hierarchy itself) in disjoint chains.
\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.8\linewidth]{resources/bip44_partition.pdf}
    \caption{%
        Chain-based partitioning of the tree defined by BIP43 and BIP44 and depicted in~\Cref{fig:resources/bip44}.
    }\label{fig:resources/bip44_partition}
\end{figure}
Each chain is a simple sequence of nodes representing users or security labels. 
Within the chain the key derivation is simple, efficient, and straightforward: 
The secret of the $i$-th element of the chain is derived directly from the secret of the $i-1$-th element, \emph{i.e.}, its predecessor in the chain.
Nodes that \emph{connect} two or more chains of the hierarchy also serve a special purpose:
They serve as intermediate nodes for the key derivation in the chain they belong to, and they also hold additional keys to \emph{bridge} the other chains that they connect to.
As an example,~\Cref{fig:resources/bip44_partition} describes a partitioning the graph of~\Cref{fig:resources/bip44}. 
The node labeled with BTC belongs to chain $0$, the chain composed of all the leftmost elements of the tree.
As such, its secret is used to derive the secret of its children labeled with $0$ belonging to the same chain.
At the same time, it connects chain $1$ of its other children, labeled with $1$, to its chain and back to the tree:
For this reason, it will hold an additional secret, \emph{i.e.}, the secret of its children labeled with $1$, to allow for the derivation of its key and of those of its descendants.
In 2015, Crampton \emph{et al.}~\cite{crampton2015} showed that there always exists an optimal chain partition of an arbitrary hierarchy and describe a polynomial algorithm to find it.
In addition, they prove that with an optimal partitioning no user is required to store more than $w$ keys, where $w$ is the number of different chains.
An efficient implementation of HKA based on chain partitioning and pseudorandom functions (PRFs) has been proposed by Freire \emph{et al.}~\cite{freire2013} in 2013.
The authors also proved the security of the scheme under key indistinguishability.

\subsection{BIP44 HDW through HKA schemes}\label{sub:hdw_through_hka_schemes}
Our first goal is to leverage chain-based hierarchical key assignment to replicate the hierarchical deterministic wallet defined in BIP44 that we described in~\Cref{sub:from_keys_to_a_tree,fig:resources/bip44}.
We recall that BIP44 defines the wallet's hierarchy with a tree where children nodes are uniquely identified by their index with respect to their parent.

We begin by partitioning the tree in disjoint chains:
We use a modified Depth-First-Search (DFS) visit that puts any children with index $0$ (\emph{i.e.}, the leftmost) in the same chain of their parent, and all the others in as many new chains.
As a result, we get exactly $w$ chains, where $w$ is the maximum branching factor of the tree.
\Cref{fig:resources/bip44_partition} describes the result of the partitioning on the hierarchy of~\Cref{fig:resources/bip44}.
Then, we leverage a slight variation of the scheme described by Freire \emph{et al.}~\cite{freire2013} to deterministically assign a secret and a key to all the elements of the tree.

More in details, each chain describes a totally ordered hierarchy.
The derivation of the secret of each node works as follows.
Let $s_0$ be a secret assigned to the first element of the chain and let $\fash$ be a pseudorandom function (in our case, $\fash_k(x) = \text{SHA3\_512}(k \concat x)$).
For each node of index $i$ in the chain and for $i > 0$, the secret $s_i$ is defined as:
\begin{equation}
    s_i = \fash_{S_{i - 1}}(0)
\end{equation}
For any node $i$, the key $k_i$ is:
\begin{equation}
    k_i = \fash_{s_{i}}(-1)
\end{equation}

To select the $s_0^j$ secrets of the $w$ chains in the partitions, we proceed as follows.
We first derive the secret of the root node of the tree, $s_0^0$, from the user's seed $S_{-1}$ (as defined by BIP32).
\begin{equation}
    s_0^0 = \fash_{S_{-1}}(0)
\end{equation}
Any other head of a chain will have exactly one predecessor, since the hierarchy is a tree.
Let $j$ be a chain and, without loss of generality, let $j - 1$ be the chain that connects the chain $j$ back to the tree. 
Let the $i$-th node of the $j - 1$-th chain be the connection node.
Let the head of chain $j$ be the $n$-th children of the $i$-th node of chain $j - 1$.
Then:
\begin{equation}\label{eq:chain_connect}
    s_0^j = \fash_{s_i^{j - 1}}(n).
\end{equation}
$n$ is always different than $0$ in~\Cref{eq:chain_connect}, since otherwise the head of the chain $j$ would be the leftmost children of its parent and our DFS would put both nodes in the same chain.

The implementation of a chain-based HKA scheme proposed by Freire \emph{et al.}~\cite{freire2013} is secure under key-indistinguishability.
There, the authors choose the secrets $S_0^j$ of any head of a chain $j$ at random.
In our case instead, we choose it deterministically by using the secret of their parent node as the key of a PRF $\fash$.
However, since the output of $\fash$ is indistinguishable from a random string of the same length, our scheme is as secure as the one proposed by Freire \emph{et al.} under the same security definitions (\emph{i.e.}, key indistinguishability).

Since we are working on a tree, our chain-based scheme can also be compactly defined as follows.
For any node $u$, being the $n$-th children of its parent $v$ (regardless of its chain and of its position in the chain):
\begin{equation}\label{eq:compact}
    s_u = \fash_{s_v}(n)
\end{equation}
In addition, we note that we are not storing any additional information in the tree and that the total number of secrets is equal to the number of nodes.

Finally, we note that our implementation defines the same hierarchical structure of BIP44 (since we work on the same tree) and benefits from the properties defined in BIP32 (specifically,~\Cref{prp:determinism} and~\Cref{prp:secret_keys});~\Cref{prp:public_keys} does not hold --- our scheme always perform the \emph{hardened} key derivation described in BIP32.

\subsection{BIP32: An instance of chain-based HKA}\label{sub:bip32_an_instance_of_chain_based_hka}
The compact representation of our scheme defined in~\Cref{eq:compact} shows how the secret of a node $u$ exclusively depends on the secret of its parent $v$ and on its index as a children $n$. 
As such, the equation shows strong similarities with how BIP32 defines the key derivation for the $n$-th child of a root node in~\Cref{eq:secret_key_h}, with the pseudorandom function $\fash_k(x)$ defined as $\hash(k \concat x) + k$.
By transitivity, the same considerations apply to the chain-based definitions of our scheme.
This result shows, intuitively, that BIP32 is a particular instance of the chain-based HKA scheme proposed first by Crampton \emph{et al.} and then by Freire \emph{et al.}~\cite{crampton2010,freire2013}.
As such, even if we do not provide formal proof, we believe that BIP32 is secure under the same security definitions (\emph{i.e.}, key indistinguishability).


==> keymall.tex <==
In this work, we are interested in signature schemes whose key pairs are malleable.
Malleability refers to the ability to transform a valid key pair $(\pk{}, \sk{})$ into a new valid one $(\pk', \sk')$ by applying respectively an operation \pkop{} on \pk{} and an operation \skop{} on \sk{}.

\begin{definition}[$(\pkop, \skop, \cXX)$-key-malleability of signatures] \label{def:keyMallSig}
	A signature scheme $\Pi= (\Keygen, \Sign, \Verify)$ is $(\pkop, \skop, \cXX)$-key-malleable if:
  \begin{enumerate}
    \item $\Pi= (\Keygen, \Sign, \Verify)$ is a standard signature scheme.
    \item For every $\secpar\in\NN$, $x \in \cXX$, there exists $r \in \cRR$ such that:
      \[
      \prob{(\pk'{},\sk'{}) = \Gen(\secparam; r)} =1,
      \]
      where $(\pk{}, \sk{}) \sample \Keygen(\secparam)$, $\pk'{} = \pk{} \pkop{} x$, $\sk'{} = \sk{} \skop{} x$, and $\cRR$ is the randomness space of the generation algorithm $\Keygen$.
  \end{enumerate}
\end{definition}

Several signatures schemes are key malleable.
As an example, DSA/ECDSA and Schnorr signatures have key pairs of the form $(\pk = \cGroupPub{y}, \sk = y)$.
It is easy to see that a valid key pair $(\cGroupPub{y}, y)$ can be transformed into a new valid key pair $(\cGroupPub{y+x}, y+x)$ by applying, with input $x$, an operation of exponentiation and multiplication on the public key and an addition operation on the secret key.

